Refining Santa: An Exercise in Efficient Synchronization

The Santa Claus Problem is an intricate exercise for concurrent programming. This paper outlines the refinement steps to develop a highly efficient implementation with concurrent objects, starting from a simple specification. The efficiency of the implementation is compared to those in other languages.

==> eptcsdata.tex <==
\providecommand{\firstpage}{68}
\providecommand{\publicationstatus}{J. Derrick, B. Dongol and S. Reeves (Eds.):\\ Refinement Workshop 2018 (REFINE'18).\\
EPTCS 282, 2018, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.282.6}{10.4204/EPTCS.282.6}}

